On an injectivity theorem for log-canonical pairs with analytic adjoint ideal sheaves

As an application of the residue functions corresponding to the lc-measures developed by the authors, the proof of the injectivity theorem on compact K\"ahler manifolds for plt pairs by Matsumura is improved in this article to allow multiplier ideal sheaves of plurisubharmonic functions with neat analytic singularities in the coefficients of the relevant cohomology groups. With the use of a refined version of analytic adjoint ideal sheaves, a plan towards a solution to the generalised version of Fujino's conjecture (i.e. an injectivity theorem on compact K\"ahler manifolds for lc pairs with multiplier ideal sheaves) is laid down and, in addition to the result for plt pairs, a proof for lc pairs in dimension 2, which is also an improvement of Matsumura's result, is given.

==> mariostdcommands.tex <==
%%%%%
%%%%% File name  : mariostdcommands.tex
%%%%% Author     : Mario Chan
%%%%% Last update: 2nd September, 2022
%%%%% Description: Math LaTeX command definitions (without packages)
%%%%%              used by Mario Chan.
%%%%%
%%
%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Begin of definitions of commands 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\newcommand{\fieldC}{\mathbb{C}}
\newcommand{\fieldR}{\mathbb{R}}
\newcommand{\fieldQ}{\mathbb{Q}}
\newcommand{\Znum}{\mathbb{Z}}
\newcommand{\Nnum}{\mathbb{N}}
\newcommand{\Nnump}{\mathbb{N}_{>0}}
%\newcommand{\Onum}{\mathfrak{o}}
%\newcommand{\Cl}{\mathscr{C}\!\mathpzc{l}}
\newcommand{\Zmod}[1]{\Znum/#1\Znum}

\newcommand{\cplxi}{\sqrt{-1}}
\newlength{\ibarbarheight}
\setlength{\ibarbarheight}{-0.9ex}
\newcommand{\ibar}{{\raisebox{\ibarbarheight}{$\mathchar'26$}\mkern-6.7mu i}}
\newcommand{\ibardefn}{\frac{\cplxi}{2\pi}}
\newsavebox{\ibarExplainBox}
\begin{lrbox}{\ibarExplainBox}
  \footnotesize
  \verb:{\raisebox{-0.9ex}{$\mathchar'26$}\mkern-6.7mu i}: 
\end{lrbox}
\newcommand{\ibarfootnote}{\footnote{The notation is chosen by
    mimicking the reduced Planck constant $\hbar = \frac{h}{2\pi}$. It
    is typeset with the code \usebox\ibarExplainBox.}}
\newcommand{\proj}{\mathbb{P}}
\newcommand{\sphere}{\mathbb{S}}
\newcommand{\uhp}{\mathfrak{H}}
\newcommand{\eps}{\varepsilon}
\newcommand{\vphi}{\varphi}

\newcommand{\sheaf}[1]{\mathscr{#1}}
\newcommand{\ideal}[1]{\mathfrak{#1}}
\newcommand{\bundle}[1]{\mathbb{#1}}

\newcommand{\mero}{\sheaf{M}}
\newcommand{\holo}{\sheaf{O}}
\newcommand{\holoform}{\boldsymbol\Omega}
\newcommand{\kanshf}[1][X]{\sheaf K_{#1}}
\newcommand{\smooth}[1][\infty]{\mathscr C^{#1}}
\NewDocumentCommand{\smform} { s D//{p,q} O{X} }{
  \sheaf A^{#2}_{#3\IfBooleanT{#1}{\,c}}  
}
\newcommand{\Lloc}[1][1]{L^{#1}_{\text{loc}}}
\newcommand{\maxidl}{\ideal m}
\newcommand{\multidl}{\sheaf I}

\NewDocumentCommand{\Tgt}{ %% Tangent bundle
  s       %% #1 turn to cotangent bundle when starred
  d//     %% #2 types of (co)tangent vectors wrt almost cplx structure
}{\mathbf T^{\IfBooleanT{#1}{*\IfNoValueF{#2}{\,}}\IfNoValueF{#2}{#2}}}

\def\cTgt{\Tgt*} %% Cotangent bundle, for backward compatibility

% \newcommand{\Tgt}[1][]{\mathbf T^{#1}}
% \newcommand{\cTgt}[1][]{\Tgt[*\,#1]}

\NewDocumentCommand{\cohgp}{
  O{H}   %% #1 symbol for cohomology (e.g.~H or \check H)
  t_     %% #2 with "_", it becomes homology
  m      %% #3 (co)homology degree
  D<>{}  %% #4 sub/super-scripts to be put to the (co)homology group
  o      %% #5 supporting space
  D//{,} %% #6 separator between space and coefficients 
  m      %% #7 coefficients
}{
  #1\IfBooleanTF{#2} {_{#3}^{#4}} {^{#3}_{#4}} \paren{\IfNoValueF{#5}{#5#6} #7}
}

\NewDocumentCommand{\cohdim}{
  t_     %% with "_", it becomes homology
  m      %% (co)homology degree
  D<>{}  %% sub/super-scripts to be put to the (co)homology group
  o      %% supporting space
  D//{,} %% separator between space and coefficients 
  m      %% coefficients
}{
  h\IfBooleanTF{#1} {_{#2}^{#3}} {^{#2}_{#3}} \paren{\IfNoValueF{#4}{#4#5} #6}
}

\newcommand{\codim}{\operatorname{codim}}
\newcommand{\Sing}{\operatorname{Sing}}
\newcommand{\mult}{\operatorname{mult}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\im}{\operatorname{im}}
\newcommand{\Res}{\operatorname{Res}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\pr}{\operatorname{pr}}
\newcommand{\Tr}{\operatorname{Tr}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\vol}{\operatorname{vol}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\Dom}{\operatorname{Dom}}
\newcommand{\Alb}{\operatorname{Alb}}
\newcommand{\alb}{\operatorname{alb}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Exc}{\operatorname{Exc}}
\newcommand{\Hess}{\operatorname{Hess}}
\newcommand{\esssup}{\operatorname*{ess\,sup}}
\newcommand{\BigO}{\operatorname{\mathbf{O}}}

% \newcommand{\bexp}{\boldsymbol{\operatorname{e}}}

\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}

\newcommand{\symmgp}{\mathfrak{S}}
\newcommand{\GL}[2][2]{\mathrm{GL}_{#1}(#2)}
\newcommand{\SL}[2][2]{\mathrm{SL}_{#1}(#2)}
\newcommand{\SO}[2][2]{\mathrm{SO}_{#1}(#2)}
% \newcommand{\SL}[1]{\mathrm{SL}_2(#1)}
% \newcommand{\SO}[1]{\mathrm{SO}_2(#1)}
\newcommand{\SU}[1]{\mathrm{SU}(#1)}
\newcommand{\Aut}[1]{\mathrm{Aut}(#1)}
\newcommand{\Div}[1]{\mathrm{Div}(#1)}
\newcommand{\divsr}[1]{\mathrm{div}\paren{#1}}

\newcommand{\sgn}[1]{\operatorname{sgn}(#1)}

%%%%% Could be replaced by calling the package "mleftright" 
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}
%%%%%

\newcommand{\lparpht}[2][(]{\mathopen{\left#1\vphantom{#2}\right.\kern-\nulldelimiterspace}}
\newcommand{\rparpht}[2][)]{\mathclose{\left.\kern-\nulldelimiterspace\vphantom{#2}\right#1}}
% \newcommand{\lparpht}[1]{\mathopen{\left(\vphantom{#1}\right.\kern-\nulldelimiterspace}}
% \newcommand{\rparpht}[1]{\mathclose{\left.\kern-\nulldelimiterspace\vphantom{#1}\right)}}
% \newcommand{\paren}[1]{\!\left(#1\right)}
\newcommand{\paren}[1]{\lparpht{#1}#1\rparpht{#1}}
\newcommand{\bigparen}[1]{\bigl(#1\bigr)}
\newcommand{\res}[1]{\left.#1\right|}
\newcommand{\parres}[1]{\res{\paren{#1}}}
\newcommand{\seq}[1]{\lparpht[\{]{#1}#1\rparpht[\}]{#1}}
% \newcommand{\seq}[1]{\left\{#1\right\}}
\newcommand{\set}[1]{\lparpht[\{]{#1}#1\rparpht[\}]{#1}}
% \newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\setd}[2]{\left\{#1\:\left|\;\vphantom{#1} #2\right.\right\}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigabs}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bignorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\Bignorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\inner}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\ptinner}[2]{\left(#1,#2\right)}
\newcommand{\biginner}[2]{\bigl\langle#1,#2\bigr\rangle}
\newcommand{\commut}[2]{\left[#1,#2\right]}
\newcommand{\algnorm}[1]{\mathbf N(#1)}
\newcommand{\smod}[1]{\,(\operatorname{mod}\,#1)}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\Ceil}[1]{\bigl\lceil#1\bigr\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\fracpart}[1]{\left\{#1\right\}}

\newcommand{\tp}[1]{\,{\vphantom{#1}}^*\! #1}
\newcommand{\rtp}[1]{\,{\vphantom{#1}}^t\! #1}

\newcommand{\genby}[1]{\left\langle#1\right\rangle}
\newcommand{\genbyd}[2]{\left\langle#1\:\left|\;\vphantom{#1} #2\right.\right\rangle}

\newcommand{\tmatrix}[4]{\left[\begin{smallmatrix}#1 & #2 \\ #3 & #4\end{smallmatrix}\right]}
\newcommand{\Diag}[1]{\operatorname{diag}\bigl(#1\bigr)}

\newcommand{\cl}{\overline}

\newcommand{\vect}[1]{\underline{#1}}

\newcommand{\conj}{\overline}
\newcommand{\diff}{\partial}
%% \dbar is defined in amsrefs (mathscinet) with out 'lite' option, so
%% \renewcommand is used 
\makeatletter
\@ifundefined{dbar}{
  \newcommand{\dbar}{{\conj\diff}}  
}{
  \renewcommand{\dbar}{{\conj\diff}}
  % \PackageWarningNoLine{marionotations}{`\protect\dbar' is redefined}
  \@latex@warning@no@line{`\protect\dbar' is redefined in mariostdcommands.tex}
}
\makeatother

\NewDocumentCommand{\fdiff}{O{#3} m O{}}{\frac{\diff #1}{\diff #2}}
\newcommand{\dfadj}{\vartheta}
\newcommand{\ddbar}{\diff\dbar}
\newcommand{\iddbar}{\cplxi\ddbar}
\newcommand{\ibddbar}{\ibar\ddbar}

\newcommand{\ddc}{dd^c\mspace{1mu}}

\newcommand{\bdry}{\partial}

\newcommand{\birat}{\mathrel{\dashrightarrow}}
\newcommand{\tendsto}{\mathrel{\rightarrow}}
\newcommand{\xtendsto}[1]{\mathrel{\xrightarrow{#1}}}
\newcommand{\wktendsto}{\mathrel{\rightharpoonup}}
\newcommand{\descendsto}{\mathrel{\searrow}}
\newcommand{\ascendsto}{\mathrel{\nearrow}}
\newcommand{\imply}{\mathrel{\Rightarrow~}}
\newcommand{\isom}{\mathrel{\cong}}
\newcommand{\ctrt}{\mathbin{\lrcorner}}


